Public Concern and the Financial Markets during the COVID-19 outbreak

We measure the public concern during the outbreak of COVID-19 disease using three data sources from Google Trends (YouTube, Google News, and Google Search). Our findings are three-fold. First, the public concern in Italy is found to be a driver of the concerns in other countries. Second, we document that Google Trends data for Italy better explains the stock index returns of France, Germany, Great Britain, the United States, and Spain with respect to their country-based indicators. Finally, we perform a time-varying analysis and identify that the most severe impacts in the financial markets occur at each step of the Italian lock-down process.

==> scaled_reg_lag15_on_IT_GoNe.tex <==
\begin{table}[H] 
\centering 
\small 
\begin{threeparttable} 
\begin{tabular}{|l|*{6}{c}|} 
\toprule 
& DE& FR& GB& US& IT& ES\\ 
\midrule 
$\alpha_i$& 0.006** & 0.004* & 0.003* & 0.006** & 0.007** & 0.006** \\ 
& (0.003) & (0.003) & (0.002) & (0.003) & (0.003) & (0.003) \\ 
$\beta_{1,i}$& 0.017* & 0.019* & 0.021* & 0.033** & 0.019 & 0.020 \\ 
& (0.012) & (0.014) & (0.014) & (0.016) & (0.020) & (0.015) \\ 
$\beta_{5,i}$& -0.042*** & -0.042*** & -0.040*** & -0.055*** & -0.052** & -0.048*** \\ 
& (0.015) & (0.016) & (0.015) & (0.018) & (0.024) & (0.018) \\ 
$\delta_i$& 0.051 & 0.050 & 0.049 & -0.129* & -0.019 & 0.025 \\ 
& (0.165) & (0.176) & (0.145) & (0.096) & (0.094) & (0.100) \\ 
& & & & & & \\ 
\midrule 
$\bar{R}^2$  & 0.055  & 0.049  & 0.048  & 0.054  & 0.061  & 0.070 \\ 
\bottomrule 
\end{tabular} 
\caption{\footnotesize Estimates of $\alpha_i$, $\beta_i$, $\delta_i$ for all countries. Social data: Google News.} 
\label{tab:reg_lag15_on_IT_GoNe} 
\begin{tablenotes}[para, flushleft] 
\item {\scriptsize Robust standard errors are in parentheses, *, ** and *** denote statistical significance at 10\%, 5\% and 1\%, respectively.} 
\end{tablenotes} 
\end{threeparttable} 
\end{table} 


==> scaled_reg_lag15_on_IT_GoSe.tex <==
\begin{table}[H] 
\centering 
\small 
\begin{threeparttable} 
\begin{tabular}{|l|*{6}{c}|} 
\toprule 
& DE& FR& GB& US& IT& ES\\ 
\midrule 
$\alpha_i$& 0.006** & 0.004** & 0.003* & 0.005** & 0.006** & 0.005** \\ 
& (0.003) & (0.002) & (0.002) & (0.003) & (0.003) & (0.003) \\ 
$\beta_{1,i}$& 0.024* & 0.028* & 0.029* & 0.036** & 0.034 & 0.030* \\ 
& (0.016) & (0.018) & (0.018) & (0.018) & (0.028) & (0.021) \\ 
$\beta_{5,i}$& -0.054*** & -0.055*** & -0.051*** & -0.061*** & -0.071** & -0.062*** \\ 
& (0.018) & (0.020) & (0.019) & (0.018) & (0.032) & (0.024) \\ 
$\delta_i$& 0.062 & 0.061 & 0.063 & -0.118 & -0.004 & 0.040 \\ 
& (0.157) & (0.166) & (0.134) & (0.094) & (0.082) & (0.085) \\ 
& & & & & & \\ 
\midrule 
$\bar{R}^2$  & 0.091  & 0.088  & 0.087  & 0.066  & 0.113  & 0.110 \\ 
\bottomrule 
\end{tabular} 
\caption{\footnotesize Estimates of $\alpha_i$, $\beta_i$, $\delta_i$ for all countries. Social data: Google Search.} 
\label{tab:reg_lag15_on_IT_GoSe} 
\begin{tablenotes}[para, flushleft] 
\item {\scriptsize Robust standard errors are in parentheses, *, ** and *** denote statistical significance at 10\%, 5\% and 1\%, respectively.} 
\end{tablenotes} 
\end{threeparttable} 
\end{table} 


==> scaled_reg_lag15_on_IT_YoTu.tex <==
\begin{table}[H] 
\centering 
\small 
\begin{threeparttable} 
\begin{tabular}{|l|*{6}{c}|} 
\toprule 
& DE& FR& GB& US& IT& ES\\ 
\midrule 
$\alpha_i$& 0.006** & 0.005** & 0.003* & 0.007** & 0.006** & 0.005** \\ 
& (0.003) & (0.002) & (0.002) & (0.003) & (0.003) & (0.003) \\ 
$\beta_{1,i}$& 0.021* & 0.023* & 0.023** & 0.018** & 0.028* & 0.024* \\ 
& (0.015) & (0.015) & (0.013) & (0.011) & (0.021) & (0.015) \\ 
$\beta_{5,i}$& -0.052*** & -0.051*** & -0.046*** & -0.048*** & -0.064*** & -0.055*** \\ 
& (0.013) & (0.014) & (0.013) & (0.009) & (0.021) & (0.015) \\ 
$\delta_i$& 0.044 & 0.045 & 0.044 & -0.141* & -0.036 & 0.022 \\ 
& (0.137) & (0.122) & (0.097) & (0.101) & (0.084) & (0.067) \\ 
& & & & & & \\ 
\midrule 
$\bar{R}^2$  & 0.122  & 0.109  & 0.104  & 0.057  & 0.127  & 0.123 \\ 
\bottomrule 
\end{tabular} 
\caption{\footnotesize Estimates of $\alpha_i$, $\beta_i$, $\delta_i$ for all countries. Social data: YouTube.} 
\label{tab:reg_lag15_on_IT_YoTu} 
\begin{tablenotes}[para, flushleft] 
\item {\scriptsize Robust standard errors are in parentheses, *, ** and *** denote statistical significance at 10\%, 5\% and 1\%, respectively.} 
\end{tablenotes} 
\end{threeparttable} 
\end{table} 


==> scaled_reg_lag15_on_IT_soc_GoNe.tex <==
\begin{table}[H] 
\centering 
\small 
\begin{threeparttable} 
\begin{tabular}{|l|*{6}{c}|} 
\toprule 
& DE& FR& GB& US& IT& ES\\ 
\midrule 
$\alpha_i$& 0.006*** & 0.004*** & 0.003*** & 0.005*** & 0.007*** & 0.006*** \\ 
& (0.003) & (0.003) & (0.002) & (0.002) & (0.003) & (0.003) \\ 
$\beta_{1,i}$& 0.016** & 0.018** & 0.020** & 0.035** & 0.020** & 0.019** \\ 
& (0.013) & (0.014) & (0.014) & (0.015) & (0.019) & (0.015) \\ 
$\beta_{5,i}$& -0.042*** & -0.043*** & -0.040*** & -0.053*** & -0.052*** & -0.048*** \\ 
& (0.014) & (0.016) & (0.015) & (0.017) & (0.023) & (0.018) \\ 
& & & & & & \\ 
\midrule 
$\bar{R}^2$  & 0.067  & 0.061  & 0.060  & 0.051  & 0.074  & 0.083 \\ 
\bottomrule 
\end{tabular} 
\caption{\footnotesize Estimates of $\alpha_i$, $\beta_i$ for all countries. Social data: Google News.} 
\label{tab:reg_lag15_on_IT_soc_GoNe} 
\begin{tablenotes}[para, flushleft] 
\item {\scriptsize Robust standard errors are in parentheses, *, ** and *** denote statistical significance at 10\%, 5\% and 1\%, respectively.} 
\end{tablenotes} 
\end{threeparttable} 
\end{table} 


==> scaled_reg_lag15_on_IT_soc_GoSe.tex <==
\begin{table}[H] 
\centering 
\small 
\begin{threeparttable} 
\begin{tabular}{|l|*{6}{c}|} 
\toprule 
& DE& FR& GB& US& IT& ES\\ 
\midrule 
$\alpha_i$& 0.006*** & 0.004*** & 0.003*** & 0.005*** & 0.006*** & 0.005*** \\ 
& (0.003) & (0.002) & (0.002) & (0.002) & (0.003) & (0.003) \\ 
$\beta_{1,i}$& 0.022** & 0.026** & 0.027** & 0.039** & 0.034** & 0.028** \\ 
& (0.018) & (0.019) & (0.018) & (0.017) & (0.028) & (0.021) \\ 
$\beta_{5,i}$& -0.054*** & -0.055*** & -0.051*** & -0.061*** & -0.071*** & -0.062*** \\ 
& (0.018) & (0.019) & (0.018) & (0.018) & (0.032) & (0.024) \\ 
& & & & & & \\ 
\midrule 
$\bar{R}^2$  & 0.101  & 0.099  & 0.097  & 0.067  & 0.126  & 0.122 \\ 
\bottomrule 
\end{tabular} 
\caption{\footnotesize Estimates of $\alpha_i$, $\beta_i$ for all countries. Social data: Google Search.} 
\label{tab:reg_lag15_on_IT_soc_GoSe} 
\begin{tablenotes}[para, flushleft] 
\item {\scriptsize Robust standard errors are in parentheses, *, ** and *** denote statistical significance at 10\%, 5\% and 1\%, respectively.} 
\end{tablenotes} 
\end{threeparttable} 
\end{table} 


==> scaled_reg_lag15_on_IT_soc_YoTu.tex <==
\begin{table}[H] 
\centering 
\small 
\begin{threeparttable} 
\begin{tabular}{|l|*{6}{c}|} 
\toprule 
& DE& FR& GB& US& IT& ES\\ 
\midrule 
$\alpha_i$& 0.007*** & 0.005*** & 0.004*** & 0.006*** & 0.006*** & 0.005*** \\ 
& (0.003) & (0.002) & (0.002) & (0.003) & (0.003) & (0.002) \\ 
$\beta_{1,i}$& 0.019** & 0.021** & 0.021** & 0.022** & 0.029** & 0.023** \\ 
& (0.017) & (0.016) & (0.014) & (0.010) & (0.021) & (0.015) \\ 
$\beta_{5,i}$& -0.052*** & -0.051*** & -0.046*** & -0.046*** & -0.064*** & -0.056*** \\ 
& (0.013) & (0.013) & (0.012) & (0.008) & (0.020) & (0.015) \\ 
& & & & & & \\ 
\midrule 
$\bar{R}^2$  & 0.133  & 0.121  & 0.115  & 0.052  & 0.139  & 0.136 \\ 
\bottomrule 
\end{tabular} 
\caption{\footnotesize Estimates of $\alpha_i$, $\beta_i$ for all countries. Social data: YouTube.} 
\label{tab:reg_lag15_on_IT_soc_YoTu} 
\begin{tablenotes}[para, flushleft] 
\item {\scriptsize Robust standard errors are in parentheses, *, ** and *** denote statistical significance at 10\%, 5\% and 1\%, respectively.} 
\end{tablenotes} 
\end{threeparttable} 
\end{table} 


==> scaled_reg_lag15_own_GoNe.tex <==
\begin{table}[H] 
\centering 
\small 
\begin{threeparttable} 
\begin{tabular}{|l|*{6}{c}|} 
\toprule 
& DE& FR& GB& US& IT& ES\\ 
\midrule 
$\alpha_i$& 0.008** & 0.003 & 0.002 & 0.005** & 0.007** & 0.003** \\ 
& (0.004) & (0.003) & (0.003) & (0.003) & (0.003) & (0.002) \\ 
$\beta_{1,i}$& 0.030** & 0.078** & 0.076** & 0.068*** & 0.019 & 0.066*** \\ 
& (0.016) & (0.035) & (0.036) & (0.018) & (0.020) & (0.021) \\ 
$\beta_{5,i}$& -0.058*** & -0.094*** & -0.089** & -0.084*** & -0.052** & -0.085*** \\ 
& (0.019) & (0.038) & (0.041) & (0.020) & (0.024) & (0.026) \\ 
$\delta_i$& 0.000 & -0.011 & -0.016 & -0.152* & -0.019 & 0.025 \\ 
& (0.174) & (0.185) & (0.178) & (0.101) & (0.094) & (0.094) \\ 
& & & & & & \\ 
\midrule 
$\bar{R}^2$  & 0.125  & 0.118  & 0.146  & 0.053  & 0.061  & 0.174 \\ 
\bottomrule 
\end{tabular} 
\caption{\footnotesize Estimates of $\alpha_i$, $\beta_i$, $\delta_i$ for all countries. Social data: Google News.} 
\label{tab:reg_lag15_own_GoNe} 
\begin{tablenotes}[para, flushleft] 
\item {\scriptsize Robust standard errors are in parentheses, *, ** and *** denote statistical significance at 10\%, 5\% and 1\%, respectively.} 
\end{tablenotes} 
\end{threeparttable} 
\end{table} 


==> scaled_reg_lag15_own_GoSe.tex <==
\begin{table}[H] 
\centering 
\small 
\begin{threeparttable} 
\begin{tabular}{|l|*{6}{c}|} 
\toprule 
& DE& FR& GB& US& IT& ES\\ 
\midrule 
$\alpha_i$& 0.003 & 0.000 & -0.001 & 0.001 & 0.006** & 0.000 \\ 
& (0.002) & (0.002) & (0.002) & (0.003) & (0.003) & (0.002) \\ 
$\beta_{1,i}$& 0.062*** & 0.101*** & 0.072** & 0.050** & 0.034 & 0.077*** \\ 
& (0.022) & (0.028) & (0.034) & (0.027) & (0.028) & (0.015) \\ 
$\beta_{5,i}$& -0.082*** & -0.112*** & -0.074** & -0.057** & -0.071** & -0.090*** \\ 
& (0.026) & (0.034) & (0.034) & (0.025) & (0.032) & (0.018) \\ 
$\delta_i$& 0.015 & -0.076 & -0.005 & -0.130 & -0.004 & 0.011 \\ 
& (0.153) & (0.146) & (0.169) & (0.113) & (0.082) & (0.102) \\ 
& & & & & & \\ 
\midrule 
$\bar{R}^2$  & 0.153  & 0.200  & 0.119  & 0.023  & 0.113  & 0.182 \\ 
\bottomrule 
\end{tabular} 
\caption{\footnotesize Estimates of $\alpha_i$, $\beta_i$, $\delta_i$ for all countries. Social data: Google Search.} 
\label{tab:reg_lag15_own_GoSe} 
\begin{tablenotes}[para, flushleft] 
\item {\scriptsize Robust standard errors are in parentheses, *, ** and *** denote statistical significance at 10\%, 5\% and 1\%, respectively.} 
\end{tablenotes} 
\end{threeparttable} 
\end{table} 


==> scaled_reg_lag15_own_YoTu.tex <==
\begin{table}[H] 
\centering 
\small 
\begin{threeparttable} 
\begin{tabular}{|l|*{6}{c}|} 
\toprule 
& DE& FR& GB& US& IT& ES\\ 
\midrule 
$\alpha_i$& 0.001 & -0.001 & -0.002 & 0.002 & 0.006** & 0.001 \\ 
& (0.003) & (0.003) & (0.003) & (0.003) & (0.003) & (0.002) \\ 
$\beta_{1,i}$& 0.051*** & 0.061*** & 0.059** & 0.051** & 0.028* & 0.074*** \\ 
& (0.021) & (0.025) & (0.030) & (0.025) & (0.021) & (0.015) \\ 
$\beta_{5,i}$& -0.064*** & -0.070** & -0.063** & -0.065*** & -0.064*** & -0.096*** \\ 
& (0.022) & (0.031) & (0.035) & (0.023) & (0.021) & (0.019) \\ 
$\delta_i$& -0.009 & -0.039 & -0.026 & -0.161* & -0.036 & -0.001 \\ 
& (0.159) & (0.156) & (0.151) & (0.096) & (0.084) & (0.087) \\ 
& & & & & & \\ 
\midrule 
$\bar{R}^2$  & 0.161  & 0.117  & 0.078  & 0.035  & 0.127  & 0.187 \\ 
\bottomrule 
\end{tabular} 
\caption{\footnotesize Estimates of $\alpha_i$, $\beta_i$, $\delta_i$ for all countries. Social data: YouTube.} 
\label{tab:reg_lag15_own_YoTu} 
\begin{tablenotes}[para, flushleft] 
\item {\scriptsize Robust standard errors are in parentheses, *, ** and *** denote statistical significance at 10\%, 5\% and 1\%, respectively.} 
\end{tablenotes} 
\end{threeparttable} 
\end{table} 


==> scaled_reg_lag15_own_soc_GoNe.tex <==
\begin{table}[H] 
\centering 
\small 
\begin{threeparttable} 
\begin{tabular}{|l|*{6}{c}|} 
\toprule 
& DE& FR& GB& US& IT& ES\\ 
\midrule 
$\alpha_i$& 0.008*** & 0.003* & 0.002 & 0.004* & 0.007** & 0.003** \\ 
& (0.003) & (0.002) & (0.002) & (0.003) & (0.003) & (0.002) \\ 
$\beta_{1,i}$& 0.030** & 0.078*** & 0.076** & 0.064*** & 0.020 & 0.065*** \\ 
& (0.017) & (0.032) & (0.034) & (0.019) & (0.019) & (0.021) \\ 
$\beta_{5,i}$& -0.058*** & -0.093*** & -0.088** & -0.077*** & -0.052** & -0.086*** \\ 
& (0.018) & (0.033) & (0.037) & (0.021) & (0.023) & (0.025) \\ 
& & & & & & \\ 
\midrule 
$\bar{R}^2$  & 0.138  & 0.132  & 0.158  & 0.045  & 0.074  & 0.185 \\ 
\bottomrule 
\end{tabular} 
\caption{\footnotesize Estimates of $\alpha_i$, $\beta_i$ for all countries. Social data: Google News.} 
\label{tab:reg_lag15_own_soc_GoNe} 
\begin{tablenotes}[para, flushleft] 
\item {\scriptsize Robust standard errors are in parentheses, *, ** and *** denote statistical significance at 10\%, 5\% and 1\%, respectively.} 
\end{tablenotes} 
\end{threeparttable} 
\end{table} 


==> scaled_reg_lag15_own_soc_GoSe.tex <==
\begin{table}[H] 
\centering 
\small 
\begin{threeparttable} 
\begin{tabular}{|l|*{6}{c}|} 
\toprule 
& DE& FR& GB& US& IT& ES\\ 
\midrule 
$\alpha_i$& 0.003* & -0.000 & -0.001 & 0.001 & 0.006** & 0.000 \\ 
& (0.002) & (0.002) & (0.002) & (0.003) & (0.003) & (0.002) \\ 
$\beta_{1,i}$& 0.062*** & 0.098*** & 0.072** & 0.048** & 0.034 & 0.077*** \\ 
& (0.022) & (0.025) & (0.031) & (0.025) & (0.028) & (0.015) \\ 
$\beta_{5,i}$& -0.082*** & -0.106*** & -0.074*** & -0.053** & -0.071** & -0.090*** \\ 
& (0.023) & (0.027) & (0.031) & (0.024) & (0.032) & (0.017) \\ 
& & & & & & \\ 
\midrule 
$\bar{R}^2$  & 0.166  & 0.207  & 0.133  & 0.021  & 0.126  & 0.194 \\ 
\bottomrule 
\end{tabular} 
\caption{\footnotesize Estimates of $\alpha_i$, $\beta_i$ for all countries. Social data: Google Search.} 
\label{tab:reg_lag15_own_soc_GoSe} 
\begin{tablenotes}[para, flushleft] 
\item {\scriptsize Robust standard errors are in parentheses, *, ** and *** denote statistical significance at 10\%, 5\% and 1\%, respectively.} 
\end{tablenotes} 
\end{threeparttable} 
\end{table} 


==> scaled_reg_lag15_own_soc_YoTu.tex <==
\begin{table}[H] 
\centering 
\small 
\begin{threeparttable} 
\begin{tabular}{|l|*{6}{c}|} 
\toprule 
& DE& FR& GB& US& IT& ES\\ 
\midrule 
$\alpha_i$& 0.001 & -0.001 & -0.002 & 0.001 & 0.006*** & 0.001 \\ 
& (0.003) & (0.002) & (0.002) & (0.003) & (0.003) & (0.002) \\ 
$\beta_{1,i}$& 0.051*** & 0.060*** & 0.058** & 0.047** & 0.029* & 0.074*** \\ 
& (0.021) & (0.022) & (0.026) & (0.026) & (0.021) & (0.015) \\ 
$\beta_{5,i}$& -0.063*** & -0.068*** & -0.062** & -0.056** & -0.064*** & -0.096*** \\ 
& (0.018) & (0.022) & (0.029) & (0.026) & (0.020) & (0.018) \\ 
& & & & & & \\ 
\midrule 
$\bar{R}^2$  & 0.173  & 0.129  & 0.091  & 0.025  & 0.139  & 0.199 \\ 
\bottomrule 
\end{tabular} 
\caption{\footnotesize Estimates of $\alpha_i$, $\beta_i$ for all countries. Social data: YouTube.} 
\label{tab:reg_lag15_own_soc_YoTu} 
\begin{tablenotes}[para, flushleft] 
\item {\scriptsize Robust standard errors are in parentheses, *, ** and *** denote statistical significance at 10\%, 5\% and 1\%, respectively.} 
\end{tablenotes} 
\end{threeparttable} 
\end{table} 


==> scaled_reg_lag_on_IT_GoNe.tex <==
\begin{table}[H] 
\centering 
\small 
\begin{threeparttable} 
\begin{tabular}{|l|*{6}{c}|} 
\toprule 
& DE& FR& GB& US& IT& ES\\ 
\midrule 
$\alpha_i$& 0.007*** & 0.006** & 0.004** & 0.009*** & 0.009*** & 0.008*** \\ 
& (0.003) & (0.002) & (0.002) & (0.003) & (0.003) & (0.003) \\ 
$\beta_i$& -0.031** & -0.030** & -0.026** & -0.037*** & -0.043** & -0.040*** \\ 
& (0.014) & (0.015) & (0.012) & (0.014) & (0.018) & (0.015) \\ 
$\delta_i$& -0.072 & -0.099 & -0.121 & -0.487*** & -0.234* & -0.239* \\ 
& (0.112) & (0.152) & (0.169) & (0.150) & (0.151) & (0.151) \\ 
& & & & & & \\ 
\midrule 
$\bar{R}^2$  & 0.058  & 0.057  & 0.053  & 0.246  & 0.115  & 0.122 \\ 
\bottomrule 
\end{tabular} 
\caption{\footnotesize Estimates of $\alpha_i$, $\beta_i$, $\delta_i$ for all countries. Social data: Google News.} 
\label{tab:reg_lag_on_IT_GoNe} 
\begin{tablenotes}[para, flushleft] 
\item {\scriptsize Robust standard errors are in parentheses, *, ** and *** denote statistical significance at 10\%, 5\% and 1\%, respectively.} 
\end{tablenotes} 
\end{threeparttable} 
\end{table} 


==> scaled_reg_lag_on_IT_GoSe.tex <==
\begin{table}[H] 
\centering 
\small 
\begin{threeparttable} 
\begin{tabular}{|l|*{6}{c}|} 
\toprule 
& DE& FR& GB& US& IT& ES\\ 
\midrule 
$\alpha_i$& 0.007*** & 0.006** & 0.005** & 0.009*** & 0.010*** & 0.008*** \\ 
& (0.003) & (0.003) & (0.002) & (0.003) & (0.004) & (0.003) \\ 
$\beta_i$& -0.040** & -0.040** & -0.035** & -0.046*** & -0.057*** & -0.051*** \\ 
& (0.017) & (0.018) & (0.015) & (0.015) & (0.023) & (0.019) \\ 
$\delta_i$& -0.090 & -0.120 & -0.137 & -0.495*** & -0.271* & -0.265* \\ 
& (0.122) & (0.162) & (0.174) & (0.154) & (0.166) & (0.166) \\ 
& & & & & & \\ 
\midrule 
$\bar{R}^2$  & 0.086  & 0.087  & 0.080  & 0.263  & 0.159  & 0.157 \\ 
\bottomrule 
\end{tabular} 
\caption{\footnotesize Estimates of $\alpha_i$, $\beta_i$, $\delta_i$ for all countries. Social data: Google Search.} 
\label{tab:reg_lag_on_IT_GoSe} 
\begin{tablenotes}[para, flushleft] 
\item {\scriptsize Robust standard errors are in parentheses, *, ** and *** denote statistical significance at 10\%, 5\% and 1\%, respectively.} 
\end{tablenotes} 
\end{threeparttable} 
\end{table} 


==> scaled_reg_lag_on_IT_YoTu.tex <==
\begin{table}[H] 
\centering 
\small 
\begin{threeparttable} 
\begin{tabular}{|l|*{6}{c}|} 
\toprule 
& DE& FR& GB& US& IT& ES\\ 
\midrule 
$\alpha_i$& 0.008*** & 0.007*** & 0.006** & 0.010*** & 0.011*** & 0.009*** \\ 
& (0.003) & (0.003) & (0.003) & (0.003) & (0.004) & (0.003) \\ 
$\beta_i$& -0.042*** & -0.041*** & -0.036*** & -0.047*** & -0.058*** & -0.051*** \\ 
& (0.014) & (0.015) & (0.012) & (0.012) & (0.021) & (0.017) \\ 
$\delta_i$& -0.123 & -0.146 & -0.166 & -0.517*** & -0.309* & -0.295* \\ 
& (0.129) & (0.166) & (0.164) & (0.152) & (0.189) & (0.187) \\ 
& & & & & & \\ 
\midrule 
$\bar{R}^2$  & 0.122  & 0.116  & 0.111  & 0.289  & 0.189  & 0.186 \\ 
\bottomrule 
\end{tabular} 
\caption{\footnotesize Estimates of $\alpha_i$, $\beta_i$, $\delta_i$ for all countries. Social data: YouTube (for Italy).}
\label{tab:reg_lag_on_IT_YoTu} 
\begin{tablenotes}[para, flushleft] 
\item {\scriptsize Robust standard errors are in parentheses, *, ** and *** denote statistical significance at 10\%, 5\% and 1\%, respectively.} 
\end{tablenotes} 
\end{threeparttable} 
\end{table} 


==> scaled_reg_lag_own_GoNe.tex <==
\begin{table}[H] 
\centering 
\small 
\begin{threeparttable} 
\begin{tabular}{|l|*{6}{c}|} 
\toprule 
& DE& FR& GB& US& IT& ES\\ 
\midrule 
$\alpha_i$& 0.009*** & 0.003 & 0.003 & 0.005* & 0.009*** & 0.007** \\ 
& (0.003) & (0.003) & (0.003) & (0.003) & (0.003) & (0.004) \\ 
$\beta_i$& -0.035*** & -0.022 & -0.020 & -0.024* & -0.043** & -0.038** \\ 
& (0.014) & (0.017) & (0.016) & (0.016) & (0.018) & (0.020) \\ 
$\delta_i$& -0.110 & -0.066 & -0.079 & -0.455*** & -0.234* & -0.249 \\ 
& (0.127) & (0.166) & (0.166) & (0.159) & (0.151) & (0.194) \\ 
& & & & & & \\ 
\midrule 
$\bar{R}^2$  & 0.102  & 0.020  & 0.018  & 0.197  & 0.115  & 0.110 \\ 
\bottomrule 
\end{tabular} 
\caption{\footnotesize Estimates of $\alpha_i$, $\beta_i$, $\delta_i$ for all countries. Social data: Google News.} 
\label{tab:reg_lag_own_GoNe} 
\begin{tablenotes}[para, flushleft] 
\item {\scriptsize Robust standard errors are in parentheses, *, ** and *** denote statistical significance at 10\%, 5\% and 1\%, respectively.} 
\end{tablenotes} 
\end{threeparttable} 
\end{table} 


==> scaled_reg_lag_own_GoSe.tex <==
\begin{table}[H] 
\centering 
\small 
\begin{threeparttable} 
\begin{tabular}{|l|*{6}{c}|} 
\toprule 
& DE& FR& GB& US& IT& ES\\ 
\midrule 
$\alpha_i$& 0.006** & 0.001 & -0.001 & 0.002 & 0.010*** & 0.003 \\ 
& (0.003) & (0.003) & (0.003) & (0.004) & (0.004) & (0.004) \\ 
$\beta_i$& -0.037** & -0.023 & -0.011 & -0.017 & -0.057*** & -0.037* \\ 
& (0.020) & (0.019) & (0.015) & (0.019) & (0.023) & (0.027) \\ 
$\delta_i$& -0.082 & -0.050 & -0.057 & -0.439*** & -0.271* & -0.220 \\ 
& (0.142) & (0.162) & (0.158) & (0.158) & (0.166) & (0.224) \\ 
& & & & & & \\ 
\midrule 
$\bar{R}^2$  & 0.054  & 0.010  & -0.011  & 0.174  & 0.159  & 0.076 \\ 
\bottomrule 
\end{tabular} 
\caption{\footnotesize Estimates of $\alpha_i$, $\beta_i$, $\delta_i$ for all countries. Social data: Google Search.} 
\label{tab:reg_lag_own_GoSe} 
\begin{tablenotes}[para, flushleft] 
\item {\scriptsize Robust standard errors are in parentheses, *, ** and *** denote statistical significance at 10\%, 5\% and 1\%, respectively.} 
\end{tablenotes} 
\end{threeparttable} 
\end{table} 


==> scaled_reg_lag_own_YoTu.tex <==
\begin{table}[H] 
\centering 
\small 
\begin{threeparttable} 
\begin{tabular}{|l|*{6}{c}|} 
\toprule 
& DE& FR& GB& US& IT& ES\\ 
\midrule 
$\alpha_i$& 0.006** & 0.002 & -0.000 & 0.005 & 0.011*** & 0.004 \\ 
& (0.003) & (0.003) & (0.003) & (0.004) & (0.004) & (0.004) \\ 
$\beta_i$& -0.032** & -0.024 & -0.014 & -0.030* & -0.058*** & -0.050* \\ 
& (0.017) & (0.021) & (0.017) & (0.021) & (0.021) & (0.033) \\ 
$\delta_i$& -0.078 & -0.059 & -0.070 & -0.469*** & -0.309* & -0.225 \\ 
& (0.139) & (0.166) & (0.159) & (0.171) & (0.189) & (0.224) \\ 
& & & & & & \\ 
\midrule 
$\bar{R}^2$  & 0.047  & 0.012  & -0.007  & 0.200  & 0.189  & 0.107 \\ 
\bottomrule 
\end{tabular} 
\caption{\footnotesize Estimates of $\alpha_i$, $\beta_i$, $\delta_i$ for all countries. Social data: YouTube (country-specific).}
\label{tab:reg_lag_own_YoTu} 
\begin{tablenotes}[para, flushleft] 
\item {\scriptsize Robust standard errors are in parentheses, *, ** and *** denote statistical significance at 10\%, 5\% and 1\%, respectively.} 
\end{tablenotes} 
\end{threeparttable} 
\end{table} 


==> scaled_reg_on_IT_GoNe.tex <==
\begin{table}[H] 
\centering 
\small 
\begin{threeparttable} 
\begin{tabular}{|l|*{6}{c}|} 
\toprule 
& DE& FR& GB& US& IT& ES\\ 
\midrule 
$\alpha_i$& 0.006*** & 0.005** & 0.004** & 0.006** & 0.007*** & 0.006** \\ 
& (0.002) & (0.002) & (0.002) & (0.003) & (0.003) & (0.003) \\ 
$\beta_i$& -0.028** & -0.027** & -0.023** & -0.025** & -0.035** & -0.032*** \\ 
& (0.013) & (0.013) & (0.011) & (0.011) & (0.016) & (0.013) \\ 
& & & & & & \\ 
\midrule 
$\bar{R}^2$  & 0.066  & 0.061  & 0.053  & 0.028  & 0.076  & 0.082 \\ 
\bottomrule 
\end{tabular} 
\caption{\footnotesize Estimates of $\alpha_i$, $\beta_i$ for all countries. Social data: Google News.} 
\label{tab:reg_on_IT_GoNe} 
\begin{tablenotes}[para, flushleft] 
\item {\scriptsize Robust standard errors are in parentheses, *, ** and *** denote statistical significance at 10\%, 5\% and 1\%, respectively.} 
\end{tablenotes} 
\end{threeparttable} 
\end{table} 


==> scaled_reg_on_IT_GoSe.tex <==
\begin{table}[H] 
\centering 
\small 
\begin{threeparttable} 
\begin{tabular}{|l|*{6}{c}|} 
\toprule 
& DE& FR& GB& US& IT& ES\\ 
\midrule 
$\alpha_i$& 0.006*** & 0.005** & 0.004** & 0.006** & 0.008*** & 0.006** \\ 
& (0.002) & (0.002) & (0.002) & (0.003) & (0.003) & (0.003) \\ 
$\beta_i$& -0.036*** & -0.036*** & -0.031*** & -0.031*** & -0.045*** & -0.040*** \\ 
& (0.014) & (0.014) & (0.012) & (0.010) & (0.019) & (0.015) \\ 
& & & & & & \\ 
\midrule 
$\bar{R}^2$  & 0.091  & 0.086  & 0.075  & 0.038  & 0.104  & 0.104 \\ 
\bottomrule 
\end{tabular} 
\caption{\footnotesize Estimates of $\alpha_i$, $\beta_i$ for all countries. Social data: Google Search.} 
\label{tab:reg_on_IT_GoSe} 
\begin{tablenotes}[para, flushleft] 
\item {\scriptsize Robust standard errors are in parentheses, *, ** and *** denote statistical significance at 10\%, 5\% and 1\%, respectively.} 
\end{tablenotes} 
\end{threeparttable} 
\end{table} 


==> scaled_reg_on_IT_YoTu.tex <==
\begin{table}[H] 
\centering 
\small 
\begin{threeparttable} 
\begin{tabular}{|l|*{6}{c}|} 
\toprule 
& DE& FR& GB& US& IT& ES\\ 
\midrule 
$\alpha_i$& 0.007*** & 0.006** & 0.005** & 0.007** & 0.008*** & 0.007** \\ 
& (0.003) & (0.003) & (0.002) & (0.003) & (0.003) & (0.003) \\ 
$\beta_i$& -0.038*** & -0.036*** & -0.031*** & -0.031*** & -0.043*** & -0.039*** \\ 
& (0.010) & (0.011) & (0.009) & (0.008) & (0.015) & (0.012) \\ 
& & & & & & \\ 
\midrule 
$\bar{R}^2$  & 0.120  & 0.109  & 0.098  & 0.047  & 0.117  & 0.120 \\ 
\bottomrule 
\end{tabular} 
\caption{\footnotesize Estimates of $\alpha_i$, $\beta_i$ for all countries. Social data: YouTube.} 
\label{tab:reg_on_IT_YoTu} 
\begin{tablenotes}[para, flushleft] 
\item {\scriptsize Robust standard errors are in parentheses, *, ** and *** denote statistical significance at 10\%, 5\% and 1\%, respectively.} 
\end{tablenotes} 
\end{threeparttable} 
\end{table} 


==> scaled_reg_own_GoNe.tex <==
\begin{table}[H] 
\centering 
\small 
\begin{threeparttable} 
\begin{tabular}{|l|*{6}{c}|} 
\toprule 
& DE& FR& GB& US& IT& ES\\ 
\midrule 
$\alpha_i$& 0.008*** & 0.003 & 0.002 & 0.004 & 0.007*** & 0.005* \\ 
& (0.003) & (0.003) & (0.003) & (0.003) & (0.003) & (0.003) \\ 
$\beta_i$& -0.031*** & -0.020* & -0.019 & -0.016* & -0.035** & -0.029** \\ 
& (0.011) & (0.015) & (0.015) & (0.012) & (0.016) & (0.017) \\ 
& & & & & & \\ 
\midrule 
$\bar{R}^2$  & 0.102  & 0.030  & 0.026  & 0.005  & 0.076  & 0.067 \\ 
\bottomrule 
\end{tabular} 
\caption{\footnotesize Estimates of $\alpha_i$, $\beta_i$ for all countries. Social data: Google News.} 
\label{tab:reg_own_GoNe} 
\begin{tablenotes}[para, flushleft] 
\item {\scriptsize Robust standard errors are in parentheses, *, ** and *** denote statistical significance at 10\%, 5\% and 1\%, respectively.} 
\end{tablenotes} 
\end{threeparttable} 
\end{table} 


==> scaled_reg_own_GoSe.tex <==
\begin{table}[H] 
\centering 
\small 
\begin{threeparttable} 
\begin{tabular}{|l|*{6}{c}|} 
\toprule 
& DE& FR& GB& US& IT& ES\\ 
\midrule 
$\alpha_i$& 0.005** & 0.001 & -0.001 & 0.001 & 0.008*** & 0.002 \\ 
& (0.003) & (0.002) & (0.003) & (0.003) & (0.003) & (0.003) \\ 
$\beta_i$& -0.033** & -0.022 & -0.011 & -0.011 & -0.045*** & -0.029* \\ 
& (0.017) & (0.018) & (0.014) & (0.016) & (0.019) & (0.021) \\ 
& & & & & & \\ 
\midrule 
$\bar{R}^2$  & 0.060  & 0.021  & 0.000  & -0.005  & 0.104  & 0.045 \\ 
\bottomrule 
\end{tabular} 
\caption{\footnotesize Estimates of $\alpha_i$, $\beta_i$ for all countries. Social data: Google Search.} 
\label{tab:reg_own_GoSe} 
\begin{tablenotes}[para, flushleft] 
\item {\scriptsize Robust standard errors are in parentheses, *, ** and *** denote statistical significance at 10\%, 5\% and 1\%, respectively.} 
\end{tablenotes} 
\end{threeparttable} 
\end{table} 


==> scaled_reg_own_YoTu.tex <==
\begin{table}[H] 
\centering 
\small 
\begin{threeparttable} 
\begin{tabular}{|l|*{6}{c}|} 
\toprule 
& DE& FR& GB& US& IT& ES\\ 
\midrule 
$\alpha_i$& 0.005** & 0.002 & -0.000 & 0.002 & 0.008*** & 0.003 \\ 
& (0.003) & (0.003) & (0.002) & (0.003) & (0.003) & (0.003) \\ 
$\beta_i$& -0.029** & -0.022 & -0.013 & -0.016 & -0.043*** & -0.041* \\ 
& (0.014) & (0.019) & (0.016) & (0.014) & (0.015) & (0.026) \\ 
& & & & & & \\ 
\midrule 
$\bar{R}^2$  & 0.054  & 0.023  & 0.003  & 0.000  & 0.117  & 0.073 \\ 
\bottomrule 
\end{tabular} 
\caption{\footnotesize Estimates of $\alpha_i$, $\beta_i$ for all countries. Social data: YouTube.} 
\label{tab:reg_own_YoTu} 
\begin{tablenotes}[para, flushleft] 
\item {\scriptsize Robust standard errors are in parentheses, *, ** and *** denote statistical significance at 10\%, 5\% and 1\%, respectively.} 
\end{tablenotes} 
\end{threeparttable} 
\end{table} 

